Resource characterisation of quantum entanglement and nonlocality in multipartite settings

Quantum technologies are enjoying an unprecedented popularity, and some applications are already in the market. This thesis studies two phenomena that are behind a lot of quantum technologies: entanglement and nonlocality. We focus on multipartite systems, and ask what configurations of those systems are more useful than others. 'Usefulness' takes on different meanings depending on the context, but, roughly speaking, we aim for more entanglement or more nonlocality. Chapter 2 develops a resource theory of entanglement with a unique multipartite maximally entangled state. Chapter 3 shows that any connected network of bipartite pure entangled states is genuine multipartite nonlocal (GMNL). Chapter 4 shows that, unlike in the case of pure states, topology is crucial to determine whether networks of bipartite mixed entangled states are genuine multipartite entangled. We also obtain, to our knowledge, the first example of superactivation of GMNL. In a departure from the main ideas explored in previous chapters, Chapter 5 is devoted to developing a physical principle inspired by a seminal result in epistemics. We contend that the principle must hold for any theory of Nature and intend for it to rule out post-quantum theories which are consistent with experimentally observed results.

==> caps/cap2.tex <==
\chapter{Planteamiento del problema}

Se pueden introducir ecuaciones de muchos tipos: 

\begin{enumerate} 
	\item En línea: $a = b$
	
	\item Numeradas
	\begin{equation}
		a = b
		\label{eq:ejemplo}
	\end{equation}
	Les podemos hacer referencia: \eqref{eq:ejemplo}.
	
	\item No numeradas
	\begin{equation*}
		a = b
	\end{equation*}
	
	\item Múltiples líneas alineadas
	\begin{align}
		a &= b \\
		c &= d + e 
	\end{align}
	
	\item Múltiples líneas alineadas, y sin número
	\begin{align*}
		a &= b \\
		c &= d + e 
	\end{align*}
	
	\item Ecuaciones en las que se distinguen casos
	\begin{equation*}
			I = 
			\begin{cases}
				1 & \textrm{si } a, \\
				0 & \textrm{si } b.
			\end{cases}
	\end{equation*}

\end{enumerate}

Todo tipo de elementos matemáticas
\begin{itemize}
		\item Fracciones $ \frac {a} {b}$ 
		
		\item Matrices 
		\begin{equation*}
			\begin{pmatrix}
				a & b \\
				c & d
			\end{pmatrix}
		\end{equation*}
\end{itemize}


\LaTeX \ permite añadir figuras:
	\begin{figure}[H]
		% Centramos la figura
		\centering
		% Anadimos el archivo de la figura, al 50% del ancho del texto
		\includegraphics[width=.5\textwidth]{fig-ejemplo}
		%% OBSERVACION
		% Las figuras se encuentran en la carpeta figuras/ 
		% añadiendo figuras en esa carpeta no es necesario poner ruta
		% tambien se pueden incluir figuras en la carpeta principal (desaconsejado)
		
		% Anadimos un texto (caption) a la figura
		\caption{Texto de la figura}
		% Y una etiqueta por si queremos hacer referencia mas adelante
		\label{fig:ejemplo}
		%% OBSERVACION
		% La etiqueta debe ser añadida DESPUES del caption.
		% Es necesario introducir un caption para que aparezca una etiqueta
		\end{figure}
Y referenciarlas: \Cref{fig:ejemplo}.\\


Normalmente el texto se estructura en secciones:

\section{Otra sección aburrida}

O incluso subsecciones

\subsubsection{Hilando fino}

O poner nombre en negrita a los párrafos:

\paragraph{Como cuestión de formato} Los saltos de línea pueden ser de 3 tipos. Sin espacios en medio e indentados, como este:

Sin espacio en medio y sin indentar, como este:
\\
O con espacio en medio e indentando, como este:\\


También podemos introducir saltos de página (aunque se desaconseja).

\pagebreak

Podemos añadir teoremas, lemas y proposiciones
\begin{thm}
	Un teorema
\end{thm}
\begin{lem}
	Un lema
\end{lem}
\begin{prop}
	Una proposición
\end{prop}
\begin{defn}
	Una definición
\end{defn}

\begin{thm}[con nombre]
	Un teorema con nombre
\end{thm}
Y citar teoremas con etiqueta
\begin{thm} \label{teo:mi teorema}
	Otro teorema
\end{thm}
Y luego lo referenciamos \Cref{teo:mi teorema}.\\

Podemos añadir citas:  \cite{cubitt+perez2015undecidability} o \cite{Bennet+Sharpley1988}. Si se añaden juntas \cite{cubitt+perez2015undecidability,Bennet+Sharpley1988}. Las referencias a sitios web también se incluirán de esta forma: \cite{LaTeXmanual}.

Para ello debemos añadir la información correspondiente al archivo \verb|bibliografia.bib| utilizando la sintaxis \verb|BibTeX|. Recomendamos el uso de Mendeley: \url{https://www.mendeley.com} para el manejo de la bibliografía. Permite almacenar pdfs y gestionar el archivo bib.\\


Podemos cargar archivos de MATLAB:
\begin{codigo}[H]
	\caption{...}
	\lstinputlisting{codigos/codigo1.m}
	\label{prog:codigo 1}
\end{codigo}
Sólo un trozo
\begin{codigo}[H]
	\caption{Línea 2 del Código \ref{prog:codigo 1}}
	\lstinputlisting[firstline=2, lastline=2]{codigos/codigo1.m}
\end{codigo}
U otros lenguajes, por ejemplo, C++
\begin{codigo}[H]
	\caption{Mi código de C++}
	\lstinputlisting[language=C++]{codigos/ejemplo.cpp}
\end{codigo}

==> caps/intro.tex <==
\chapter{Introduction}


Aquí iría la introducción del trabajo.\\

Esto es un ejemplo de texto. Se pueden enumerar items con puntos
\begin{itemize}
\item \textbf{ITEM 1}: Y lo que diga

\item\textbf{ITEM 2}: Y lo que diga

\end{itemize}

En este trabajo nos centraremos en el estudio de este último problema. \\


También se puede enumerar
\begin{itemize}

\item Una cosa otra

\item Y otra cosa

\end{itemize}

Example paragraph:

According to the first postulate of quantum mechanics, the state of
a system is described by a density operator $\rho\in\mathcal{B}(\mathcal{H})$,
the set of bounded operators on a Hilbert space $\mathcal{H}$. Vectors
on $\mathcal{H}$ are denoted by $\ket{\cdot}$, while $\bra{\cdot}$
denotes their duals. States $\rho$ must be positive and have unit
trace. If a density operator $\rho$ is a projector, i.e. $\rho^{2}=\rho$
or, equivalently, $\tr\rho^{2}=1$, the system is said to be in a
\emph{pure} state. In this case, the unit vector $\ket{\psi}\in\mathcal{H}$
such that $\rho=\ketbra{\psi}$ is sufficient to describe the state
of the quantum system, and vectors are often used in place of projective
operators. We use $\psi\equiv\ketbra{\psi}$ whenever a state is specified
as pure. Otherwise, the \emph{mixed} state $\rho$ can be written
as a probabilistic mixture of pure states,
\begin{equation}
\rho=\sum_{i\in I}p_{i}\ketbra{\psi_{i}},
\end{equation}
where $I$ is an index set, often omitted from the notation, and $\{p_{i}\}_{i\in I}$
is a probability distribution, i.e., $0\leq p_{i}\leq1$ for all $i\in I$,
and $\sum_{i\in I}p_{i}=1$.

States are often written in terms of the \emph{computational basis},
represented symbolically as \sloppy $\{\ket{0},\ket{1},...,\ket{d-1}\}$.
Each $\ket{i},i=0,...,d-1$, is a column vector with a 1 in the $(i+1)$th
position and 0 on the rest.


==> clases/bibliografia.tex <==
% Para que la bibliografia salga en indice
\addcontentsline{toc}{chapter}{\bibname}

% Formato de la bibliografia
\bibliographystyle{amsalpha}

% Archivo de la bibliografia (bibliografia/referencias.bib)
\bibliography{bibliografia/entnonloc}
